Photocurrents of charge and spin in single-layer Fe$_3$GeTe$_2$

In the realm of two-dimensional materials magnetic and transport properties of a unique representative $-$ Fe$_3$GeTe$_2$ $-$ attract ever increasing attention. Here, we use a developed first-principles method for calculating laser-induced response to study the emergence of photo-induced currents of charge and spin in single-layer Fe$_3$GeTe$_2$, which are of second order in the electric field. We provide a symmetry analysis of the emergent photocurrents in the system finding it to be in excellent agreement with ab-initio calculations. We analyse the magnitude and behavior of the charge photocurrents with respect to disorder strength, frequency and band filling. Remarkably, not only do we find a large charge current response, but also predict that Fe$_3$GeTe$_2$ can serve as a source of significant laser-induced spin-currents, which makes this material as a promising platform for various applications in optospintronics.

==> commands.tex <==
%====================================================
%MAKRO NAMES
%====================================================

\newcommand{\gfxpath}[1]{../gfx/#1}

\newcommand{\pgi}{Peter Gr\"unberg Institut and Institute for Advanced Simulation,
Forschungszentrum J\"ulich and JARA, 52425 J\"ulich, Germany}

\newcommand{\aachen}{Department of Physics, RWTH Aachen University, 52056 Aachen, Germany}

\newcommand{\mainz}{Institute of Physics, Johannes Gutenberg University Mainz, 55099 Mainz, Germany}

%====================================================
%NOTATIONS
%====================================================

%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}[theorem]
%\newtheorem{lemma}[theorem]{Lemma}
%\DeclareMathOperator*{\moyal}{\bigstar}

\newcommand{\moyal}{\bigstar}
\newcommand{\Pf}{\mathcal{P}_\mathrm{F}}
\newcommand{\pf}{P_\mathrm{F}}

\newcommand{\Algebra}{\mathbb{A}_\hbar}
\newcommand{\algebra}{\mathbb{A}_0}

\newcommand{\realdim}{d}
\newcommand{\phasespace}{\mathbb{R}^{2\realdim}}

\newcommand{\Conn}{\mathcal{A}}
\newcommand{\Curv}{\mathcal{F}}
\newcommand{\conn}{A}
\newcommand{\curv}{F}

\newcommand{\PH}{\mathbb{P}\mathcal{H}}
\newcommand{\ph}{\mathbb{P}H}

\newcommand{\qgeom}{Q}
\newcommand{\qmetric}{g}
\newcommand{\Qgeom}{\mathcal{Q}}
\newcommand{\Qmetric}{\mathrm{g}}

\newcommand{\ad}{\mathrm{ad}}

\newcommand{\cov}{\nabla}



\newcommand{\abinitio}{$ab\; initio$ }

%====================================================
%VECTORS
%====================================================

%Standard vector command
\renewcommand{\vec}[1]{\mathbf{#1}} 

%Normalized unit vector
\newcommand{\hatn}{\hat{\mathbf{n}}}

%Cartesian unit vectors
\newcommand{\xvec}{ \hat{\mathbf{e}}_x}
\newcommand{\yvec}{ \hat{\mathbf{e}}_y}
\newcommand{\zvec}{ \hat{\mathbf{e}}_z}
\newcommand{\ivec}{ \hat{\mathbf{e}}_i}

%Spherical unit vectors
\newcommand{\rvec}{ \hat{\mathbf{e}}_r}
\newcommand{\thetavec}{ \hat{\mathbf{e}}_\theta}
\newcommand{\phivec}{ \hat{\mathbf{e}}_\phi}

%Cylindrical unit vectors
\newcommand{\rhovec}{ \hat{\mathbf{e}}_\rho}
\newcommand{\varphivec}{ \hat{\mathbf{e}}_\varphi}

%Moyal diagrams
\newcommand{\diagram}[2]{\raisebox{-.0\height}{\includegraphics[scale=1]{../gfx/moy/o#1/o#1d#2.pdf}}}
\newcommand{\smalldiagram}[2]{\raisebox{-.0\height}{\includegraphics[scale=0.7]{../gfx/moy/o#1/o#1d#2.pdf}}}
\newcommand{\smallnediagram}[2]{\raisebox{-.0\height}{\includegraphics[scale=0.7]{../gfx/moy_ne/o#1/o#1d#2.pdf}}}

%Sphere
\newcommand{\sphere}{\raisebox{-.35\height}{\includegraphics[scale=0.04]{../gfx/symbols/sphere.png}}}

%====================================================
%GENERAL MATH OPERATIONS
%====================================================

%braidning
\newcommand{\braid}{\mathrm{Braid}}
\newcommand{\abraid}{\overline{\mathrm{Braid}}}

%residue
\newcommand{\Res}[1]{
\underset{#1}{\mathrm{Res}~}
}

%c numer
\newcommand{\cnumber}{c~\text{number}}

%Absolute value
\newcommand{\abs}{\mathrm{\abs}}
%Wigner transformation
\newcommand{\wigner}{\mathcal{W}}

%image space
\newcommand{\im}{\mathrm{im}}
\newcommand{\rank}{\mathrm{rank}~}

%Reduced Moyal product
\newcommand{\rstar}{\star_\mathrm{r}}

%Left-Right Partial Tensors
\newcommand{\lpartial}{\overset{\leftarrow}{\partial}}
\newcommand{\rpartial}{\overset{\rightarrow}{\partial}}
\newcommand{\lrpartials}{\overset{\leftarrow}{\boldsymbol{\partial}}\colon\!\mathrm{\reflectbox{$\overset{\leftarrow}{\boldsymbol{\partial}}$}}}
\newcommand{\rlpartials}{\overset{\rightarrow}{\boldsymbol{\partial}}\colon\!\mathrm{\reflectbox{$\overset{\rightarrow}{\boldsymbol{\partial}}$}}}

%Unitar transformation
\newcommand{\U}{\mathcal{U}}
\newcommand{\Ud}{\mathcal{U}^\dagger}

%Trace Operation
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\Tr}{\mathrm{Tr}}

%Fracture Trace Operation
\newcommand{\fraktr}{\mathfrak{Tr}}

%Diagonal matrix
\newcommand{\diag}{\mathrm{diag}}

%Sign Function
\newcommand{\sgn}{\mathrm{sgn}}

%Identity Operation
\newcommand{\id}{\mathrm{id}}

%Encircled Moyal Star Operator
\newcommand{\circdstar}{\raisebox{-.28\height}{\includegraphics[height=0.167in]{../gfx/math/circdstar.pdf}}}

%Differential d
\newcommand{\dd}{\mathrm{d}}

%Equivalent by partial integration
\newcommand{\equivpi}{\overset{\mathrm{P.I.}}{\sim}}

%Defined as /  From definition
\newcommand{\defi}{\overset{\mathrm{def}}{=}}

%Sec hyp
\newcommand{\sech}{\mathrm{sech}}

%gradient
\newcommand{\grad}{\mathrm{grad}~}

%interior product
\newcommand{\interior}{\mathrm{i}}

%====================================================
%LATTICES
%====================================================

\newcommand{\volume}{\mathcal{V}}

%====================================================
%SUSCEPTIBILITY
%====================================================

%Landau Peierls Susceptibility
\newcommand{\lp}{\chi_\mathrm{LP}}

%Orbital Magnetic Susceptibility
\newcommand{\oms}{\chi_\mathrm{oms}}

%====================================================
%ORBITAL MAGNETIZATION
%====================================================

%Orbital moment
\newcommand{\morbbf}{\mathbf{m}_\mathrm{orb}}

%Orbital magnetization (OM)
\newcommand{\ombf}{\mathbf{m}_\mathrm{om}}
\newcommand{\om}{m_\mathrm{om}}

%Topological orbital magnetization (TOM)
\newcommand{\tombf}{\mathbf{m}_\mathrm{tom}}
\newcommand{\tom}{m_\mathrm{tom}}
\newcommand{\Tom}{M_\mathrm{tom}}

%Chiral orbital magnetization (COM)
\newcommand{\combf}{\mathbf{m}_\mathrm{com}}
\newcommand{\com}{m_\mathrm{com}}
\newcommand{\Com}{M_\mathrm{com}}

\newcommand{\chiLP}{\chi_\mathrm{LP}^{\uparrow + \downarrow}}
\newcommand{\mass}{m_\mathrm{e}}

%====================================================
%GREEN'S FUNCTIONS & MATSUBARA FORMALISM
%====================================================

%normalordering
\newcommand{\norder}[1]{: #1 :}

%wick timeordering
\newcommand{\torder}{\mathcal{T}}

\newcommand{\Corder}[1]{
	\mathcal{T}_\mathrm{c}
	\left[
	#1
	\right]
}


%Keldysh space Green's function
\newcommand{\Gk}{\underline{G}}

%Retarded Green's function
\newcommand{\Gret}{G^{\mathrm{R}}}

%Advanced Green's function
\newcommand{\Gadv}{G^{\mathrm{A}}}

%Lesser Green's function
\newcommand{\Gles}{G^<}

%Causal Green's function
\newcommand{\Gcau}{G^{\mathrm{C}}}

%Matsubara energy
\newcommand{\maten}{ \xi_n}

%Matsubara frequency
\newcommand{\matfreq}{ i \omega_n}

%====================================================
%IMPORTANT KET STATES
%====================================================

\newcommand{\fockket}{\ket{\lbrace n_q\rbrace_q}}
\newcommand{\fockbra}{\ket{\lbrace n_q\rbrace_q}}

%====================================================
%PHYSICAL CONSTANTS & OPERATORS
%====================================================

%time order operator
\newcommand{\tordering}{\mathcal{T}}

%electron mass
\newcommand{\emass}{m_\mathrm{e}}

%bold pi (canonical momentum)
%\newcommand{\bpi}{\boldsymbol{\pi}}

%Vector of Pauli matrices
\newcommand{\bsigma}{\boldsymbol{\sigma}}

%Vector of Pauli matrices (alternative notation)
%\newcommand{\btau}{\boldsymbol{\tau}}

%Exchange parameter
\newcommand{\xc}{\Delta_{\mathrm{xc}}}

%Superconducting parameter
\newcommand{\superc}{\Delta_{\mathrm{sc}}}

%fermi velocity
\newcommand{\vf}{v_\mathrm{F}}

%Rashba parameter
\newcommand{\soi}{\alpha_{\mathrm{R}}}

%Vector Rashba parameter
\newcommand{\vsoi}{\boldsymbol{\alpha}_{\mathrm{R}}}

%Boltzmann constant
\newcommand{\boltzmann}{k_\mathrm{B}}
\newcommand{\kB}{\boltzmann}

%Torque operators
\newcommand{\btorque}{\mathbf{T}}
\newcommand{\torque}{T}

%Quantum Many body field  annihilation operator
\newcommand{\qfield}{\Psi}

%====================================================
%ELECTROMAGNETISM & GAUGE FIELDS
%====================================================

%Non-Abelian vector potential
\newcommand{\apotcal}{\boldsymbol{\mathcal{A}}}

%Non-Abelian field tensor
\newcommand{\ftenscal}{\mathcal{F}}

%Classical vector potential
\newcommand{\apot}{\vec{A}}

%Magnetic field
\newcommand{\bfield}{\mathbf{B}}

%Electric field
\newcommand{\efield}{\mathbf{E}}

%Magnetization

\newcommand{\magbf}{\mathbf{m}}
\newcommand{\Magbf}{\mathbf{M}}

%====================================================
%Relativity
%====================================================
\newcommand{\spacetime}{{\mathbb{R}^{1,d}}}

%====================================================
%Fourier transformation
%====================================================
\newcommand{\fourier}[1]{
	\mathcal{F}
\left[
 #1
\right]
}

%====================================================
%TEXTMODE OPERATIONS
%====================================================

\newcommand{\kspace}{$\mathbf{k}$-space}
\newcommand{\DMI}{Dzyaloshinskii-Moriya}
\newcommand{\todo}[1]{(\textcolor{red}{TODO: #1})}
\newcommand{\remark}[1]{\textcolor{blue}{#1}}
\newcommand{\new}[1]{\textcolor{blue}{#1}}
\newcommand{\proved}[1]{(\textcolor{red}{PROVED: #1})}

